Generative Motion Infilling From Imprecisely Timed Keyframes

Keyframes are a standard representation for kinematic motion specification. Recent learned motion-inbetweening methods use keyframes as a way to control generative motion models, and are trained to generate life-like motion that matches the exact poses and timings of input keyframes. However, the quality of generated motion may degrade if the timing of these constraints is not perfectly consistent with the desired motion. Unfortunately, correctly specifying keyframe timings is a tedious and challenging task in practice. Our goal is to create a system that synthesizes high-quality motion from keyframes, even if keyframes are imprecisely timed. We present a method that allows constraints to be retimed as part of the generation process. Specifically, we introduce a novel model architecture that explicitly outputs a time-warping function to correct mistimed keyframes, and spatial residuals that add pose details. We demonstrate how our method can automatically turn approximately timed keyframe constraints into diverse, realistic motions with plausible timing and detailed submovements.

==> desiderata.tex <==
\section{Design Goals}
\label{desiderata}

Our goal is to support detailing of simple character animation. As described in Sec~\ref{prelim}, our system takes as input a blocking motion \blocking. It generates a detailed motion \detailed adhering to the following desiderata:

\begin{itemize}
    \item \textit{Realistic}. \blocking lacks detail; \detailed should contain detail such that it looks like a plausible human motion.
    \item \textit{Non-destructive}. Though lacking detail, \blocking provides a guide for the desired motion and tells the story of the action. Therefore, \detailed should minimally semantic aspects of \blocking. For example, if \blocking contains a single punch, ideally \detailed does not contain a series of jabs. 
\end{itemize}

These goals may conflict in interesting ways. To add detail to a motion where a character stands on one foot and pivots, the system may have to add additional transitional movement, running against the goal of being as non-destructive to the original sequence as possible. 
